Flares, wind and nebulae: the 2015 December mini-outburst of V404 Cygni

After more than 26 years in quiescence, the black hole transient V404 Cyg went into a luminous outburst in June 2015, and additional activity was detected in late December of the same year. Here, we present an optical spectroscopic follow-up of the December mini-outburst, together with X-ray, optical and radio monitoring that spanned more than a month. Strong flares with gradually increasing intensity are detected in the three spectral ranges during the ~10 days following the Swift trigger. Our optical spectra reveal the presence of a fast outflowing wind, as implied by the detection of a P-Cyg profile (He I - 5876 A) with a terminal velocity of ~2500 km/s. Nebular-like spectra -- with an H_alpha equivalent width of ~500 A -- are also observed. All these features are similar to those seen during the main June 2015 outburst. Thus, the fast optical wind simultaneous with the radio jet is most likely present in every V404 Cyg outburst. Finally, we report on the detection of a strong radio flare in late January 2016, when X-ray and optical monitoring had stopped due to Sun constraints.

==> def_bibtex.tex <==
\def\apj{ApJ}
\def\mnras{MNRAS}
\def\aap{A\&A}
\def\apjl{ApJ}
\def\pasj{PASJ}
\def\nat{Nature}
\def\iaucirc{IAU Circ.}
\def\skytel{S\&T}
\def\aaps{A\&A S.S.}
\def\apss{Ap\&SS}
\def\apjs{ApJS}
\def\araa{ARA\&A}
\def\pasp{PASP}
